The relationship between IGM Lyman-alpha opacity and galaxy density near the end of reionization

Observed scatter in the Lyman-alpha opacity of quasar sightlines at $z<6$ has motivated measurements of the correlation between Ly$\alpha$ opacity and galaxy density, as models that predict this scatter make strong and sometimes opposite predictions for how they should be related. Our previous work associated two highly opaque Ly$\alpha$ troughs at $z\sim5.7$ with a deficit of Lyman-$\alpha$ emitting galaxies (LAEs). In this work, we survey two of the most highly transmissive lines of sight at this redshift, towards the $z=6.02$ quasar SDSS J1306+0356 and the $z=6.17$ quasar PSO J359-06. We find that both fields are underdense in LAEs within 10 $h^{-1}$ Mpc of the quasar sightline, somewhat less extensive than underdensities associated with Ly$\alpha$ troughs. We combine our observations with three additional fields from the literature, and find that while fields with extreme opacities are generally underdense, moderate opacities span a wider density range. The results at high opacities are consistent with models that invoke UV background fluctuations and/or late reionization to explain the observed scatter in IGM Ly$\alpha$ opacities. There is tension at low opacities, however, as the models tend to associate lower IGM Ly$\alpha$ opacities with higher densities. Although the number of fields surveyed is still small, the low-opacity results may support a scenario in which the ionizing background in low-density regions increases more rapidly than some models suggest after becoming ionized. Elevated gas temperatures from recent reionization may also be making these regions more transparent.

==> scratch.tex <==
%Models attempting to explain these fluctuations have appealed to large-scale variations in the ionizing UV background and/or gas temperature, and possibly ongoing reionization with large remaining neutral islands.  Notably, these models make predictions for the relationship between opacity and density that are possible to test observationally. In the first type of model, large-scale fluctuations in the UVB are the cause of the scatter. Generally, in these models a highly transmissive sightline is expected to be in close proximity to ionizing sources, whereas a highly opaque sightline would be associated with a void. There are galaxy-driven versions of this model \citep{davies16,nasir20} and quasar-driven models \citep{chardin15,chardin17}. We note that because quasars are rare, in this model \lya\ opacity is less tightly coupled to density than it is in galaxy-driven UVB models. The quasar-driven model has also been disfavored because the observed number density of quasars is not high enough to produce the required number of ionizing photons for quasars to be the main sources driving reionization \citep{mcgreer18}. Additionally, a quasar-driven hydrogen reionization may be incompatible with current constraints on helium reionization \citep{daloisio17,mcgreer18,garaldi19}.

%The second type is the temperature model, which features large-scale fluctuations in temperature \citep{daloisio15}. In this model, a highly transmissive region would be hot and recently reionized, whereas an opaque region would have reionized early and been cooling for longer. This model is disfavored by the observations of  \citet{becker18,kashino20,christenson21}, who found that highly opaque quasar sightlines are associated with galaxy underdensities.

%The last type of model employs ``ultra-late'' reionization.  These models commonly feature UVB fluctuations but are distinct from pure UVB models in that reionization continues below $z = 6$.  In the ultra-late reionization models, a highly opaque quasar sightline may correspond to a neutral island. Transmissive sightlines, however, are less straightforward; \citet{keating20b} argue that highly transmissive regions should correspond to regions that are underdense with galaxies but have recently been reionized, while \citet{nasir20} find that highly transmissive sightlines correspond to a range of galaxy densities.


%however, observations of highly opaque sightlines are not able to distinguish between galaxy UVB models and late reionization models, which both predict that highly opaque sightlines should correspond to a galaxy underdensity.  Observations over a range of \lya\ opacity are necessary to best understand how well the models do or don't agree with the data. \citet{ishimoto22} also survey two quasar sightlines of moderate opacity, SDSS J1137+3549 and SDSS J1602+4228, which display overdensities but are neither opaque nor transmissive enough to distinguish between the models. Observations of highly transmissive sightlines are needed to assess the galaxy UVB models, which predict that highly transmissive sightlines should be overdense. A set of observations spanning both opacity extremes is necessary to completely test predictions from reionization models, and further can be used to characterize the $z\sim 5.7$ opacity-density relationship, which can also be compared to model predictions.

For each model, simulated LAE populations around these sightlines are used to construct an expected surface density profile for highly transmissive lines of sight, which we compare to our measurements.


\begin{figure*}
\includegraphics[width=\textwidth]{figures/maps-globalnorm.pdf}
\caption{Distribution of LAE candidates in the J0148 field (highly opaque, top left), the J1250 field (highly opaque, top right), the J1306 field (highly transmissive, bottom left) and J359 field (highly transmissive, bottom right). As in Figure \ref{fig:lae_map}, the LAE candidates are assigned a color that indicates their $NB816$ magnitude. The grayscale shading in the background indicates the surface density of LAE candidates, which we calculate by kernel density estimation. Portions masked out of the field in white are obscured by foreground stars. Here, contrary to in Figure \ref{fig:lae_map}, the surface density is normalized by the global mean surface density measured over all four fields. The field is centered on the quasar position, which is marked with a gold star, and the concentric dotted rings indicate 10 $h^{-1}$ Mpc intervals from the quasar position. The solid ring marks the edge of the field, 45\arcmin\ from the quasar position. The contours indicate regions that are overdense relative to the global surface density mean.}
\label{fig:maps-globalnorm}
\end{figure*}
